Reducing the parameter space for Unparticle-inspired models using white dwarf masses

Based on astrophysical constraints derived from Chandrasekhar's mass limit for white-dwarfs, we study the effects of the model on the parameters of unparticle-inspired gravity, on scales $\Lambda_U > 1 \; TeV$ and $d_U \approx 1$.

==> bibliography.bib.tex <==
@Book{bib:chandrasekhar_1967,
	author = {Chandrasekhar, S.},
	title = {Introduction to the Study of Stellar Structure},
	publisher = {Dover},
	year = {1967},
	edition = {3}
}

@BOOK{bib:karttunen,
  AUTHOR = "Karttunen, H.",
  TITLE = "Fundamental Astronomy",
  YEAR = "2006",
  PUBLISHER = "Springer",
}

@BOOK{bib:carroll,
  AUTHOR = "Ostlie, D. A. and Carrol, B. W.",
  TITLE = "Modern Stellar Astrophysics",
  YEAR = "1996",
  PUBLISHER = "Addison-Wesley"
}

@Book{bib:maciel_1999,
	author = {Maciel, Walter J.},
	title = {Introdução à Estrutura e Evolução Estelar},
	publisher = {Edusp},
	year = {1999},
	edition = {1}
}

@Book{bib:camenzind_2007,
	author = {Max Camenzind},
	title = {Compact Objects in Astrophysics: White Dwarfs, Neutron Stars and Black Holes},
	publisher = {Springer-Verlag},
	year = {2007},
	edition = {1}
}

@Book{bib:shapiro_1983,
	author = {Stuart Shapiro and Saul Teukolsky},
	title = {Black Holes, White Dwarfs and Neutron Stars : The Physics of Compact Objects},
	publisher = {Wiley-Interscience},
	year = {1983},
	edition = {1}
}

@Book{bib:kepler_2003,
	author = {Kepler de Souza Oliveira Filho and Maria de Fátima Oliveira Saraiva},
	title = {Astronomia e Astrofísica},
	publisher = {Livraria da Física},
	year = {2003},
	edition = {1}
}

@ARTICLE{bib:1961ApJ...134..669S,
   author = {{Salpeter}, E.~E.},
    title = "{Energy and Pressure of a Zero-Temperature Plasma.}",
  journal={The Astrophysical Journal},
     year = 1961,
    month = nov,
  volume={134},
    pages = {669-+},
      doi = {10.1086/147194},
   adsurl = {http://adsabs.harvard.edu/abs/1961ApJ...134..669S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{bib:salpeter_1961,
  author={Hamada T. and Salpeter, E.E.},
  title={Models for Zero-Temperature Stars},
  journal={The Astrophysical Journal},
  volume={134},
  pages={683},
  year={1961}
}

@Book{bib:hansen_2004,
	author = {H., Carl J. and K., Steven D. and T., Virginia },
	title = {Stellar interiors: physical principles, structure, and evolution},
	publisher = {Springer-Verlag},
	year = {2004},
	edition = {2}
}

@ARTICLE{bib:1931MNRAS..91..456C,
	author = {{Chandrasekhar}, S.},
	title = "{The highly collapsed configurations of a stellar mass}",
	journal = {Monthly Notices of the Royal Astronomical Society},
	year = 1931,
	month = mar,
	volume = 91,
	pages = {456-466},
	adsurl = {http://adsabs.harvard.edu/abs/1931MNRAS..91..456C},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bib:1935MNRAS..95..207C,
	author = {{Chandrasekhar}, S.},
	title = "{The highly collapsed configurations of a stellar mass (Second paper)}",
	journal = {Monthly Notices of the Royal Astronomical Society},
	year = 1935,
	month = jan,
	volume = 95,
	pages = {207-225},
	adsurl = {http://adsabs.harvard.edu/abs/1935MNRAS..95..207C},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Book{bib:huang_yu_1998,
	author = {R.Q., Huang. and K.N., Yu},
	title = {Stellar Astrophysics},
	publisher = {Springer-Verlag},
	year = {1998},
	edition = {1}
}

@Book{bib:cox_vol_2_1998,
	author = {J.P., Cox and R.T., Giuli},
	title = {Principles of Stellar Structure},
	publisher = {Gordon-Breach},
	year = {1968},
	volume = {2},
	edition = {1}
}

@Book{bib:horvath_2011,
	author = {Horvath, J.E.},
	title = {Fundamentos da evolução estelar, Supernovas e Objetos Compactos},
	publisher = {Livraria Editora da Física},
	year = {2011},
	edition = {1}
}

@article{bib:0004-637X-494-2-759,
  author={J. L. Provencal and H. L. Shipman and Erik Høg and P. Thejll},
  title={Testing the White Dwarf Mass-Radius Relation with Hipparcos},
  journal={The Astrophysical Journal},
  volume={494},
  number={2},
  pages={759},
  url={http://stacks.iop.org/0004-637X/494/i=2/a=759},
  year={1998}
}
	

@Book{bib:vitensse_2011,
	author = {Böhm-Vitense, E.},
	title = {Introduction to Stellar Astrophysics},
	publisher = {Cambridge University Press},
	year = {1992},
	volume={2},
	edition = {1}
}


@article{bib:1982ApJ...256..247B,
  author={Brunish, W. M. and Truran,J. W. },
  title={The evolution of massive stars. I - The influence of mass loss on Population 1 stars},
  journal={The Astrophysical Journal},
  volume={256},
  number={1},
  pages={247-258},
  url={http://adsabs.harvard.edu/abs/1982ApJ...256..247B},
  year={1982}
}
	
@Article{bib:paxton_2010, 
	journal={The Astrophysical Journal Supplement Series},
	volume={192},
	number={1},
	year = {2011},
	author    = {Bill Paxton and Lars Bildsten and Aaron Dotter and Falk Herwig and Pierre Lesaffre and Frank Timmes}, 
	title     = {Modules for Experiments in Stellar Astrophysics (MESA)}, 
	eprint    = {astro-ph.SR/1009.1622v1}, 
	SLACcitation  = "%%CITATION = ASTRO-PH.SR 1009.1622v1;%%"
}

@Online{bib:ezweb_2011,
author = {Townsend, Rich},
title = {EZ-Web},
month = {dez},
year = {2011},
url = {http://www.astro.wisc.edu/~townsend/static.php?ref=ez-web}
}

@Book{bib:prialnik_2000,
	author = {Prialnik, Dina},
	title = {An introduction to the theory of stellar structure and evolution},
	publisher = {Cambridge University Press},
	year = {2000},
	edition = {1}
}

@Article{bib:georgi_2007,
	author    = {H. Georgi},
	title     = {Unparticle Physics},
	journal   = {Phys. Rev. Lett.},
	volume    = {98},
	year      = {2007},
	url    = {arXiv:hep-ph/0703260v3}
}

@ARTICLE{bib:kikuchi-2008-665,
  author = {Tatsuru Kikuchi and Nobuchika Okada},
  title = {Unparticle Dark Matter},
  journal = {PHYS.LETT.B},
  volume = {665},
  pages = {186},
  url = {doi:10.1016/j.physletb.2008.06.021},
  year = {2008}
}

@article{bib:PhysRevLett.100.031803,
  journal = {Phys. Rev. Lett.},
  numpages = {4},
  month = {Jan},
  doi = {10.1103/PhysRevLett.100.031803},
  issue = {3},
  author = {Goldberg, Haim and Nath, Pran},
  title = {Scalar Modifications to Gravity from Unparticle Effects May Be Testable},
  year = {2008},
  publisher = {American Physical Society},
  pages = {031803},
  volume = {100}
}

@Article{bib:bertolami_2009,
  title = {Astrophysical constraints on unparticle-inspired models of gravity},
  author = {Bertolami, O.  and P\'aramos, J.  and Santos, P. },
  journal = {Phys. Rev. D},
  volume = {80},
  number = {2},
  pages = {022001},
  numpages = {4},
  year = {2009},
  month = {Jul},
  doi = {10.1103/PhysRevD.80.022001},
  publisher = {American Physical Society}
}

@ARTICLE{bib:2007MNRAS.375.1315K,
   author = {{Kepler}, S.~O. and {Kleinman}, S.~J. and {Nitta}, A. and {Koester}, D. and 
	{Castanheira}, B.~G. and {Giovannini}, O. and {Costa}, A.~F.~M. and 
	{Althaus}, L.},
    title = "{White dwarf mass distribution in the SDSS}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0612277},
 keywords = {white dwarfs},
     year = 2007,
    month = mar,
   volume = 375,
    pages = {1315-1324},
      doi = {10.1111/j.1365-2966.2006.11388.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.375.1315K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{bib:landau_1965,
  title={Collected papers of L.D. Landau},
  author={Landau, L.D.},
  year={1965},
  publisher={Pergamon Press}
}

@article{bib:PhysRevLett.99.141301,
  author = {Davoudiasl, Hooman},
  volume = {99},
  journal = {Phys. Rev. Lett.},
  month = {Oct},
  numpages = {4},
  title = {Constraining Unparticle Physics with Cosmology and Astrophysics},
  year = {2007},
  doi = {10.1103/PhysRevLett.99.141301},
  issue = {14},
  publisher = {American Physical Society},
  pages = {141301}
}

@article{bib:1126-6708-2007-12-033,
  author={Ayres Freitas and Daniel Wyler},
  title={Astro unparticle physics},
  journal={Journal of High Energy Physics},
  volume={2007},
  number={12},
  pages={033},
  year={2007}
}
	
@article{bib:Deshpande2008888,
title = "Long range forces and limits on unparticle interactions",
journal = "Physics Letters B",
volume = "659",
number = "5",
pages = "888 - 890",
year = "2008",
issn = "0370-2693",
doi = "10.1016/j.physletb.2007.12.018",
author = "N.G. Deshpande and Stephen D.H. Hsu and Jing Jiang"
}

@article{bib:JR2008561,
title = "Unparticle-enhanced black holes at the LHC",
journal = "Physics Letters B",
volume = "660",
number = "5",
pages = "561 - 566",
year = "2008",
note = "",
issn = "0370-2693",
doi = "10.1016/j.physletb.2008.01.050",
author = "J.R. and Mureika"
}


  	
@article{bib:1475-7516-2009-03-019,
  author={John McDonald},
  title={Cosmological constraints on unparticles as continuous mass particles},
  journal={Journal of Cosmology and Astroparticle Physics},
  volume={2009},
  number={03},
  pages={019},
  year={2009}
}
	
